Axiomatic Explainer Globalness via Optimal Transport

Explainability methods are often challenging to evaluate and compare. With a multitude of explainers available, practitioners must often compare and select explainers based on quantitative evaluation metrics. One particular differentiator between explainers is the diversity of explanations for a given dataset; i.e. whether all explanations are identical, unique and uniformly distributed, or somewhere between these two extremes. In this work, we define a complexity measure for explainers, globalness, which enables deeper understanding of the distribution of explanations produced by feature attribution and feature selection methods for a given dataset. We establish the axiomatic properties that any such measure should possess and prove that our proposed measure, Wasserstein Globalness, meets these criteria. We validate the utility of Wasserstein Globalness using image, tabular, and synthetic datasets, empirically showing that it both facilitates meaningful comparison between explainers and improves the selection process for explainability methods.

==> tables/transform_table.tex <==
\begin{table}[t]
    %------------------------------------------
    % \setlength{\belowcaptionskip}{-15pt}
    % \scriptsize
    % \vspace{4mm}
    \small
    \setlength{\tabcolsep}{2.3pt}
    % \renewcommand{\arraystretch}{1.1}
    \centering
    \begin{tabular}{l l c c c c} 
    \toprule
     \multicolumn{2}{c}{\bf{Transformation}}& $\boldsymbol{\hat G_2}$ \bf{(Ours)} & \bf{SE} & \bf{KL} & \bf{TV} \\ 
     \midrule
     \emph{Isometric} \\
     \cmidrule{1-2}
     A) Identity & $t(x) = x$ & $0.43$ & $2.09$ & $29.4$ & $0.71$\\ 
     B) Reflection  & $t(x) = -x$& $0.43$ & $2.09$ & $\textcolor{red}{\boldsymbol{10.0}}$ & $0.71$\\ 
     C) Translation  & $t(x) = x+12$& $0.43$ & $2.09$ & $29.5$ & $0.71$\\ 
     \\
     \emph{Non-Isometric} \\
     \cmidrule{1-2}
     D) Absolute Value  & $t(x) = |x|$& $0.60$ & $\textcolor{red}{\boldsymbol{2.09}}$ & \bf{\textcolor{red}{DNE}} & $\textcolor{red}{\boldsymbol{0.71}}$\\ 
     \bottomrule
    \end{tabular}
    \vspace{-5mm}
\end{table}

==> tables/wasserstein_globalness_table.tex <==

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{lcc}
    \toprule 
    \textbf{Explainer} & \textbf{MNIST} & \textbf{CIFAR-10}\\
        \midrule 
         Gradients & 0.536 $\pm$ 0.027 & 0.312 $\pm$ 0.021\\
        % \hline
        SmoothGrad & 0.700 $\pm$ 0.040 & 0.328 $\pm$ 0.037 \\
        % \hline
        Guided Backprop & 0.635 $\pm$ 0.044 & 0.375 $\pm$ 0.042 \\
        % \hline
        Integrated Gradients & 0.712 $\pm$ 0.048 & 0.331 $\pm$ 0.042\\
        % \hline
        Deep-SHAP & 0.625 $\pm$ 0.029 & 0.320 $\pm$ 0.025\\
        % \hline
        Smooth Guided Backprop & 0.758 $\pm$ 0.044 & 0.352 $\pm$ 0.045 \\
        \bottomrule
    \end{tabular}
    \caption{Wasserstein Globalness for both datasets. We present the mean and standard deviation \textit{across sample neighborhoods}.}
    \label{tab:my_label}
\end{table*}
